Enhancing Natural Language Representation with Large-Scale Out-of-Domain Commonsense

We study how to enhance text representation via textual commonsense. We point out that commonsense has the nature of domain discrepancy. Namely, commonsense has different data formats and is domain-independent from the downstream task. This nature brings challenges to introducing commonsense in general text understanding tasks. A typical method of introducing textual knowledge is continuing pre-training over the commonsense corpus. However, it will cause catastrophic forgetting to the downstream task due to the domain discrepancy. In addition, previous methods of directly using textual descriptions as extra input information cannot apply to large-scale commonsense. In this paper, we propose to use large-scale out-of-domain commonsense to enhance text representation. In order to effectively incorporate the commonsense, we proposed OK-Transformer (\underline{O}ut-of-domain \underline{K}nowledge enhanced \underline{Transformer}). OK-Transformer effectively integrates commonsense descriptions and enhances them to the target text representation. In addition, OK-Transformer can adapt to the Transformer-based language models (e.g. BERT, RoBERTa) for free, without pre-training on large-scale unsupervised corpora. We have verified the effectiveness of OK-Transformer in multiple applications such as commonsense reasoning, general text classification, and low-resource commonsense settings.

==> ok_related.tex <==
\section{Related Work}


{\bf Commonsense reasoning} is considered to be a challenging task in natural language processing~\cite{levesque2012winograd}. With the development of unsupervised language models in recent years~\cite{devlin2018bert,peters2018deep,radford2019language}, people realized that commonsense can be derived from them. For example, \cite{petroni2019language} found that we can extract structured factual knowledge (e.g. ConceptNet~\cite{liu2004conceptnet}) from unsupervised language models. \cite{weir2020existence} found that the unsupervised language model implicitly represents concepts and its associated properties. In some follow-up work, researchers found that language models can be used to solve the task of commonsense-based reference disambiguation. This is also the main task that this paper focuses on.

Zero-shot's commonsense reasoning of unsupervised language models aims to study how to design algorithms to better extract commonsense from unsupervised language models. For example, \cite{trinh2018simple} found that we can use the joint probability of the sentence provided by the language model to determine whether a sentence conforms to commonsense. The author believes that sentences with high joint probability are more in line with commonsense. Therefore, the author completes the disambiguation by replacing the original pronoun with the candidate reference, and using the joint probability as the score of the sentence. Several subsequent works have used similar ideas. \cite{klein2019attention} uses the attention-guided method to calculate the score. \cite{tamborrino2020pre} uses a larger language model Roberta~\cite{liu2019roberta}, and calculates the scores of candidate sentences based on the masked word probability. \cite{shwartz2020unsupervised} provides additional clues for using generative language models (i.e. GPT-2~\cite{radford2019language}) for the target task. These works have achieved good results on some commonsense reasoning tasks.

However, \cite{zellers2019hellaswag} found that the language model is actually looking for sentences that are more in line with lexical cues, rather than sentences that are more in line with commonsense. We agree with the viewpoint of \cite{zellers2019hellaswag}. Since the language model learns and represents the association of the text and its context, this is an inevitable result of a lot of commonsense not being written directly (\cite{gordon2013reporting}). Since the representation learning of the language model is based on data association, it only models ID data, but cannot effectively represent OOD data. We believe that introducing commonsense into the language model is the only way for the language model to understand OOD data. This is also the main research direction of this article.

In contrast to the commonsense reasoning of the zero-shot unsupervised language model, some works believe that the current limitation of commonsense reasoning lies in the lack of relevant training data. Therefore, some data sets similar to common commonsense reasoning were constructed. The earliest data set similar to WSC is WSCR~\cite{rahman2012resolving}. \cite{kocijan19acl} found that if the unsupervised language model is fine-tuning on similar reference disambiguation data sets, the effect of the language model on commonsense-based reference disambiguation can be improved. Therefore, the author constructs MaskedWiki~\cite{kocijan19acl} and WikiCREM~\cite{kocijan2019wikicrem} through masking of Wikipedia data. \cite{sakaguchi2019winogrande} constructed the WinoGrande data set, which has improved WSC in terms of scale and difficulty. Some language models themselves also add such data sets to pre-training corpus. For example, Roberta's pre-training corpus STORIES~\cite{trinh2018simple} is a corpus similar to WSC. These datasets have indeed improved the effectiveness of specific commonsense reasoning tasks.

However, it is clear that the construction of these commonsense data sets is for specific tasks. Its essence is to expand the scope of the model's ID data. But the corpus is always limited. We believe that the introduction of larger data sets cannot solve the OOD problem of more general tasks. We believe that the introduction of task-independent commonsense data is the general way to solve the OOD problem.

{\bf Incorporating External Knowledge into Language Representation Learning} 

